Large Language Models for Data Annotation and Synthesis: A Survey

Data annotation and synthesis generally refers to the labeling or generating of raw data with relevant information, which could be used for improving the efficacy of machine learning models. The process, however, is labor-intensive and costly. The emergence of advanced Large Language Models (LLMs), exemplified by GPT-4, presents an unprecedented opportunity to automate the complicated process of data annotation and synthesis. While existing surveys have extensively covered LLM architecture, training, and general applications, we uniquely focus on their specific utility for data annotation. This survey contributes to three core aspects: LLM-Based Annotation Generation, LLM-Generated Annotations Assessment, and LLM-Generated Annotations Utilization. Furthermore, this survey includes an in-depth taxonomy of data types that LLMs can annotate, a comprehensive review of learning strategies for models utilizing LLM-generated annotations, and a detailed discussion of the primary challenges and limitations associated with using LLMs for data annotation and synthesis. Serving as a key guide, this survey aims to assist researchers and practitioners in exploring the potential of the latest LLMs for data annotation, thereby fostering future advancements in this critical field.

==> sections/A2.tex <==
% \documentclass[../LLM4Annotate.tex]{subfiles}

% \begin{document}
\vspace{-1mm}
\section{LLM-Generated Annotations Utilization}
\vspace{-2mm}
The LLM-generated annotations provide a valuable resource of labeled data for diverse machine learning tasks. This section explores the methodologies in learning with LLM-Generated Annotations.

\subsection{Target Domain Inference: Direct Utilization of Annotations}
In this section, we explore the practical application of LLM-generated annotations in diverse downstream tasks. Annotations, extracted from LLMs through carefully designed prompts, provide valuable predictions for a wide range of downstream applications. Such usage can be categorized according to the definitions in Section 2: a. Supervised: Labels are utilized in any form. b. Unsupervised: Annotations function as predictions with no labels involved, e.g., zero-shot scenarios.

\noindent\textbf{Predicting Labels.}
Utilizing manually designed prompts, LLMs generate predicted labels in two distinct manners. First, they predict labels while considering demonstration samples, denoted as $\hat{y}=\mathcal{A}(q(x|\sD))$. Second, they make predictions without reliance on demonstration samples, represented as $\hat{y}=\mathcal{A}(q(x))$. Depending on the source of these demonstration samples, which could be either $\sD \subset \sD_l$ or $\sD \subset \sD_u$, this can be classified as either supervised or unsupervised~\cite{sorensen2022information}. This technique has enabled LLMs to contribute to a wide array of tasks, spanning across areas such as reasoning, knowledge bases, causal reasoning, recommendation systems, healthcare, and even vision-language models~\cite{wei2022emergent, kojima2022large, petroni2019language, kiciman2023causal, hou2023large, gu2023systematic}.

\noindent\textbf{Inferring Additional Attributes.}
Similarly, LLMs adeptly correlate prompts with specific attributes or concepts, effectively in both supervised and unsupervised settings~\cite{sorensen2022information}.
 This capacity proves particularly advantageous in the case of models such as Concept Bottleneck Models~\cite{tan2023interpreting}, which generate predictions by identifying the underlying concepts. In this context, LLMs effectively tackle the issue of limited dataset annotations. In vision-language tasks, LLMs can be employed to automatically generate textual descriptions for image classifications~\cite{radford2021learning, menon2022visual}.
\vspace{-2mm}
\subsection{Knowledge Distillation: Bridging LLM and task-specific models}
Expanding on the previous discussion regarding the direct use of annotations, Knowledge Distillation (KD) emerges as an additional approach to harness the capabilities of LLMs. KD facilitates the transfer of expertise from a larger ``teacher'' model, typically an LLM, to a smaller, more focused ``student'' model. This technique enables the student model to match or even surpass the teacher's performance, despite lower resource demands.
% Formally, when presented with a dataset $\sD_{g} = \{x_k, o_k, (y_k)\}_{k=1}^R$ annotated by the teacher model $\gA$, the student model $\gL$ is trained to absorb this knowledge through learning from $\sD_{g}$.

\noindent\textbf{Model Enhancement.} Currently, several studies have embraced KD to enrich a task-specific learner model, denoted as $\gL$, with insights from an LLM-based annotator, referred to as $\gA$. For example, research endeavors like \cite{magister2022teaching, fu2023specializing, sun2023chatgpt} focus on training $\gL$ using datasets annotated by $\gA$. Conversely, \cite{hsieh2023distilling} employs ``task hardship'' as auxiliary labels supplied by $\gA$ to enhance the learning process for $\gL$. Notably, Alpaca~\cite{alpaca} and GPT4All~\cite{anand2023gpt4all} employ LLM-generated corpora to train their lightweight student models to achieve impressive  performance.

\noindent\textbf{KD Innovations.} In terms of tools, GKD~\cite{tan2023gkd} stands out as a recently developed library that simplifies the KD process with LLMs. Advancements in this dynamic field encompass both black-box~\cite{jiang2023lion} and white-box~\cite{gu2023knowledge} LLMs serving as teacher models, improvements in efficiency~\cite{jha2023large}, and expansions into specialized domains such as biomedical knowledge extraction~\cite{gu2023distilling}, code generation~\cite{gunasekar2023textbooks}, web content filtering~\cite{voros2023web}, and mathematical reasoning~\cite{fu2023specializing}.

\noindent In summary, the adoption of KD for training task-specific models offers the dual advantages of decreased computational demands and sustained performance, positioning it as a highly promising avenue in contemporary natural language processing.

\vspace{-1mm}
\subsection{Harnessing LLM Annotations for Fine-Tuning and Prompting}

The use of LLM-generated annotations for fine-tuning or prompting in LLM adaptation is increasingly popular, following Knowledge Distillation principles to unlock LLMs' potential. Studies show that larger datasets for supervised fine-tuning enhance LLMs' generalization~\cite{sanh2021multitask, wei2021finetuned}, highlighting the growing importance of LLM-annotated data~\cite{wang2022super}. These methods mainly fall into four categories:\\
\noindent\textbf{In-Context Learning.}
Originating from the GPT-3 model~\cite{brown2020language}, In-Context Learning (ICL) has been widely employed to boost the performance of LLMs across varied tasks. The approach often employs specially formatted prompts that include task instructions along with illustrative demonstrations~\cite{dong2022survey}. These prompts assist LLMs in extrapolating to new, unseen tasks without requiring explicit parameter updates. Although effective, 
%%%%%although these additional prompts (including instructions and demonstrations) have proven effective for various tasks, 
they are generally difficult to achieve~\cite{margatina2023active}. Therefore, an effective approach to obtaining helpful prompts based on the annotations generated by LLMs~\cite{hongjin2022selective}. As the task instructions are crucial for the performance of ICL, multiple works are proposed to automatically generate instructions without the laborious process of human manipulations~\cite{zhao2023survey}. In~\cite{honovich2022instruction}, the authors observe that provided with several demonstration examples, LLMs can learn to generate the instructions for various tasks and thus promote ICL performance. 
%%%%%Automatic Prompt Engineer (APE)~\cite{liu2021makes,lee2022does} is proposed to automatically generate instructions and also perform the selection of beneficial. In particular, APE regards the instruction as the ``program'', which is optimized by searching through a set of instruction candidates suggested by an LLM to maximize a specific score function. 
Apart from methods that utilize LLM-generated annotations as instructions, other works also explore the possibility of leveraging LLM-generated demonstrations for ICL~\cite{dong2022survey}. Among them, a recent work named synthetic prompting~\cite{shao2023synthetic} has gained traction. This technique constructs new questions based on a given input question's reasoning chain, followed by a clustering method to select the most diversified and complex demonstrations. Utilizing raw text datasets as a warm up, \cite{chen2022improving} introduce a method to create self-supervised data that aligns with ICL learning formats for various downstream tasks. 
%%%%%In particular, the authors convert raw text into input-output pairs and investigate four self-supervised objectives, encompassing masked token prediction and various classification tasks.\\

\noindent\textbf{Chain-of-Thought Prompting.}
It represents a specialized method within ICL that specifically enhances the performance of LLMs on intricate reasoning tasks like arithmetic reasoning~\cite{miao2021diverse}, common-sense reasoning~\cite{talmor2018commonsenseqa}, and symbolic reasoning~\cite{wei2022chain}. Unlike traditional ICL, 
%which chiefly involves the generation of input-output pairs for prompting,
CoT introduces intermediate reasoning steps in the prompts. These steps are designed to contribute meaningfully toward the final output. This distinction underscores the focus of CoT on the mechanics of reasoning.
%%%%%, whereas ICL typically concentrates on example selection and ordering. 
It is widely evaluated that creating effective CoT prompts is crucial for unlocking LLMs' intricate reasoning capabilities~\cite{dong2022survey}. As manual creation of such prompts can be costly and time-consuming~\cite{wei2022chain}, recent works have prevalently proposed to automatically generate CoT prompts via LLMs. For example, in Zero-shot CoT~\cite{kojima2022large}, LLMs are prompted with ``Let's think step by step'' to generate reasoning steps, followed by ``Therefore, the answer is'' to reach the conclusion. Auto-CoT~\cite{zhang2022automatic} refines this approach by applying a clustering strategy to the training questions to determine the most representative ones for each cluster. 
%%%%%Self-consistency~\cite{wang2022self} introduces a novel decoding strategy that aims to generate multiple reasoning paths before automatically selecting the most confident answer. 
A related study~\cite{wang2022rationale} extends this by taking into account prompt confidence, finding that diverse reasoning paths are essential for effective CoT. In another vein, \cite{fu2023specializing} propose to combine LLM-generated CoT and few-shot demonstrations to preserve ICL capabilities while enhancing the reasoning performance on using different prompt formats. \cite{wang2023scott} explore the use of LLM-annotated rationales for knowledge distillation based on CoT prompting. 
Despite irrelevant or vacuous rationales, authors use contrastive decoding to significantly improve the reasoning abilities of student models trained with this augmented data.

\noindent\textbf{Instruction Tuning.}
While ICL adapts LLMs by altering the input structure, instruction tuning takes a different approach by fine-tuning models on various tasks in a supervised learning context~\cite{zhao2023survey}.
%%%%%%, often employing sequence-to-sequence loss function. 
Multiple works have demonstrated that LLMs displayed notable capabilities in generalizing to unfamiliar tasks after fine-tuning~\cite{chung2022scaling,muennighoff2022crosslingual}. 
%%%%%Recent works point out that the quality of data used for fine-tuning is crucial for enhancing the generalizability of LLMs~\cite{zhou2023lima}. 
However, the process of obtaining high-quality training data for Instruction Tuning generally involves a large amount of human effort, which can be impractical in specific real-world scenarios~\cite{lou2023prompt}. To avoid the laborious process of acquiring human annotations, recent works have resorted to LLM-generated annotations.
%%%%%and also provided a deeper understanding of instruction tuning. 
As a classic example, in Self-Instruct~\cite{wang2022self}, the LLM is prompted to autonomously generate new instructional input-output pairs. These are subsequently filtered and used for the fine-tuning of a T5 model~\cite{brown2020language}. This two-stage pipeline generates instructions, filters out invalid or redundant instances, and employs the rest for model fine-tuning. Alpaca~\cite{taori2023stanford} leverages LLM-generated annotations in the form of instruction-following demonstrations to fine-tune a LLaMA model~\cite{touvron2023llama}. 
Notably, the GopherCite model~\cite{menick2022teaching} introduces a reinforcement learning framework to train LLMs to generate annotations in the form of answers supported by cited evidence, thereby enhancing the verifiability of their responses. \cite{chiang2023can} present a study on the reliability of using LLM-generated annotations for human-like evaluations across various NLP tasks. 
%%%%%The authors scrutinize the stability and consistency of evaluations generated by LLMs, comparing them with expert human assessments in contexts such as open-ended story generation and adversarial attacks.\\

\noindent\textbf{Alignment Tuning.}
Alignment tuning aims to eliminate the undesirable behaviors of LLms by aligning them with human expectations~\cite{zhao2023survey}. 
%%%%%The alignment tuning of LLMs largely relies on fine-tuning LLMs with human feedback, generally in the form of human preferences among given responses~\cite{dai2023can}. 
However, in practice, collecting human feedback can be usually expensive and laborious~\cite{ziegler2019fine}. Therefore, existing works typically learn a surrogate reward model that can imitate human preference in a pair of inputs (pairwise feedback). 
%%%%%In this manner, researchers can utilize the reward output provided by the reward model to perform alignment tuning with the LLM-generated annotations. 
To train a reward model for annotations, researchers will generally first collect a labeled pairwise feedback dataset from human annotators. Then based on different strategies, many algorithms directly learn from $\sD_l$~\cite{keskar2019ctrl, liu2023chain,korbak2023pretraining}, while other algorithms~\cite{christiano2017deep, ouyang2022training} learn a surrogate reward model from $\sD_l$ and use it to automatically annotate unlabeled pairwise feedback generated by LLMs. 
To align LLMs with annotations, existing works generally leverage the strategy of reinforcement learning~\cite{openai2023gpt4, touvron2023llama2}, namely RLHF (reinforcement learning from human feedback). As a classic example, InstructGPT~\cite{ouyang2022training} utilizes the PPO strategy~\cite{schulman2017proximal}, and in each update computes the Kullback–Leibler (KL) divergence between the current LLM output and that from the previous update. In this way, the framework can be optimized in a more robust manner. On the other hand, ILQL~\cite{snell2022offline} explores the application of alignment tuning on LLM-generated annotations under an offline setting in contrast to the prevalent online RL scenario. In GopherCite~\cite{menick2022teaching}, the authors employ reinforcement learning from human preferences (RLHP) to train QA models that produce answers and simultaneously cite specific evidence to support their claims, thereby facilitating the evaluation of accuracy. More recently, RLAIF~\cite{lee2023rlaif} leverages preferences that 
are labeled by an off-the-shelf LLM in lieu of
humans, which achieves similar performance with using human-labeled data.


% \end{document}
